Quality Assurance Challenges for Machine Learning Software Applications During Software Development Life Cycle Phases

In the past decades, the revolutionary advances of Machine Learning (ML) have shown a rapid adoption of ML models into software systems of diverse types. Such Machine Learning Software Applications (MLSAs) are gaining importance in our daily lives. As such, the Quality Assurance (QA) of MLSAs is of paramount importance. Several research efforts are dedicated to determining the specific challenges we can face while adopting ML models into software systems. However, we are aware of no research that offered a holistic view of the distribution of those ML quality assurance challenges across the various phases of software development life cycles (SDLC). This paper conducts an in-depth literature review of a large volume of research papers that focused on the quality assurance of ML models. We developed a taxonomy of MLSA quality assurance issues by mapping the various ML adoption challenges across different phases of SDLC. We provide recommendations and research opportunities to improve SDLC practices based on the taxonomy. This mapping can help prioritize quality assurance efforts of MLSAs where the adoption of ML models can be considered crucial.

==> conclusion.tex <==
% \section{Conclusions} \label{sec:conclusion}
% Many of the recent studies shows that ML models are vulnerable to various attacks, they can be stolen and misled into doing unintended things. These weaknesses have profound implications to ML applications in safety-critical applications such as self-driving cars, healthcare. Additionally some studies also points out that ML models unintentionally infer inappropriate correlations between societal biases (gender, race) from the data. A reliable machine learning system should have the ability to resist adversaries, protect user privacy and help to make pro-social decisions. The systems performance and reliability needs to be ensured when updating the ML models. The reliability and trustworthiness are compromised if the new models introduces new issues. So, experts both multiple domains such as SE, Security, NLP, computer vision should collaborate to set the foundation of trustworthy ML systems. There are open search opportunities to develop useful tools and metrics to understand them. We should more research on integrating ML research into Software applications. Ensuring the quality of MLSA is the first step towards that.

==> discussions.tex <==
% \section{Discussions} \label{sec:discussion}


==> related-work.tex <==
% \section{Related Work} \label{sec:related_work}
% % Related work \cite{Pane-MoreNatureEUSE-Springer2006}

% Roscher et. al. \cite{roscher2020explainable} discusses on the transparency, explainability, and interpretability  of ML applications with respect to natural science.

==> tables.tex <==

\begin{table*}[t]
  \centering
  %\vspace{-.1in}
   \caption{Current challenges of quality assurance in machine learning applications comparer to traditional applications}
  % \vspace{-3mm}
    % \resizebox{\columnwidth}{!}{%
    \begin{tabular}{p{0.15\textwidth}p{0.07\textwidth}p{0.60\textwidth} p{0.40\textwidth}}
    \toprule{}
    \textbf{Challenge type} & \textbf{ML stage} & \textbf{ Summary of current QA challenges } & \textbf{ Opportunities QA for MLSA }  \\
    
    
    \midrule
    \textbf{System requirement} & \\
    Ambiguous reqmt  & Reqmt &
    ML applications usually have a conceptual description of the goal rather than functional description.
    % Unlike traditional applications,  ML applications usually have a conceptual description of the goal rather than functional description. It is data driven and different understanding of data leads to the discovery of different application requirement\cite{ml_practice_2019}. During the requirement analysis, all the stakeholders should have a clear understanding to what extends ML applications can help to solve business problem \cite{ml_practice_2019}. 
    &
    Develop necessary tools, metrics for requirement analysis\cite{}.
    \\

    
    
    Standardized reporting  &  Reqmt &
    MLSA application do not have a standard reporting specification like other industries (transportation, aviation, pharmaceuticals). 
    % ML application should have some standard body like other technologies such as W3C, ISO, RIA. ML applications should also release audit trails and analysis tools for third party verification. 
    &
    Developing analysis tools for third party verification and specification for audit trails.
    % ML application should have some standard body like other technologies such as W3C, ISO, RIA. ML applications should also release audit trails and analysis tools for third party verification.
    \\
    

    

    \midrule
    \textbf{Design and planning} &  \\

    
    Social fairness  & Reqmt &
    If the data contains biases against any social, racial and genders then that needs to be address. An ML systems should fair, accountable and transparent \cite{mehrabi2019survey}. 
    &
    Develop specs for fairness \cite{gooden2015race}\cite{mehrabi_fairness_survey_2019} and tools (Themis\cite{galhotra2017fairness}).
    

    \\
    
    Privacy constraint & reqmt & 
    Many companies also can not use raw user-data because of terms and service agreement with the users, organizational legal and ethical constrains. Inability to understand the internal representation of the model might cause privacy breach \cite{castelvecchi2016can}. Federated learning\cite{mcmahan2017communication} has the potential to deliver these features without diminishing user experience and privacy \cite{li2020federated}.
    &
    There are still many open research opportunities to improve the federated learning and increase user privacy\cite{li2020federated}.
    % such as improving communication scheme, federal learning for unlabelled data,  granular privacy constraints etc  \cite{li2020federated}.
    
    % Privacy preserving models & Reqmt &
    % Inability to understand the internal representation of the model might cause privacy breach \cite{castelvecchi2016can}. On the other hand, if an adversary can guess the model's inner relation then privacy can be violated. Data privacy should be ensure throughout the entire life cycle of the ML application. Many companies also can not use raw user-data because of terms and service agreement with the users.
    % & 
    %  Federated learning \cite{mcmahan2017communication} is a potential solution for the privacy, ownership problem. It is a distributed machine learning approach that facilities to train models on remote devices such as mobile phone, remote data-centers on data without compromising privacy\cite{bonawitz2019towards}. The model can use anonymized or aggregated statistics of the raw sensitive data \cite{tata2017quick} to develop powerful predictive applications\cite{hard2018federated}. There are still many open research opportunities to improve the federated learning and increase user privacy such as improving communication scheme, federal learning for unlabelled data,  granular privacy constraints etc  \cite{li2020federated}.
    \\
    
    Regulation & Reqmt &
    During training we need to consider user data privacy, confidential data such as location, medical history. Organizations need to comply with user data protection acts HIPPA\cite{annas2003hipaa}, GDPR\cite{voigt2017eu}
    &
    Research on transparent and trustworthy AI.
    
    \\
    
    Organizational culture &  All &
    It is important to encourage team culture to adopt best ML practices such as complexity reduction, deletion of features, improving reproducibility, sharing data\cite{ml_practice_2019} by merging best of SE and ML research world\cite{sculley_hiddent_debt_2015}.
    &
    Empirical study to understand the organization and cultural aspect ML development.
    
    
    % It is important to encourage team culture to adopt best ML practices such as complexity reduction, deletion of features, improving reproducibility by merging best of SE and ML research world \cite{sculley_hiddent_debt_2015}. Qualitative and quantitative studies of developers survey suggest that different teams an organization  should promote culture to share more resources like labelled data: data curated for one task in an organization should be shared with other teams as it is a costly time consuming process\cite{ml_practice_2019}. There should be proper training and knowledge sharing options because there are usually different types of engineers from varied background and varied level of expertise in ML 
    % &
    \\
    
    
    \midrule
    \textbf{Implementation } &  \\
    
    Data management  & Data proc. &
    Data is very important for ML systems because of its garbage in garbage out nature. There is a lack of tools to manage different attributes of data such as data freshness, accuracy, structuredness, data granularity or imbalanced dataset &
    Develop tools for ML specific data management.
    \\
    
    Reusability   & Feat. Eng. &
    % Model customizability and modularity.
    % A model trained for a particular task can be reused to solve a similar problem of the same domain using transfer learning\cite{survey_transfer_learning_2009}.
    It requires a significant effort to reuse a model if the target problem is of different domain or different input format. Customizable modular design helps to ensure quality in the long run.
    % A machine learning model consists of algorithm whose parameters are trained on data. Customizing a ML model is challenging because is developed in a modular, uncoupled way like a traditional software \cite{amershi_se_case_study_2019}. A model trained for a particular task can be reused to solve a similar problem of the same domain using transfer learning\cite{survey_transfer_learning_2009}. However it requires a significant effort if the target problem is of different domain or different input format.
    &
    Transfer learning\cite{survey_transfer_learning_2009} and Model modularization\cite{pan2020decomposing}.
    \\
    

    
    Development efficiency  &  Evaluation &
    The performance of a model can not be evaluated until training on the whole dataset is finished which is Computationally expensive and time consuming.
    &
    Better ML architecture to train with less computation power.
    \\
    
    Evaluation metrics  & Evaluation &
    Evaluation metrics should be in the context where it will be applied. There are lack of tools to compare the performance of different models. 
    &
    Develop necessary tools.
    \\
 
    Data dependency  & All &
    ML applications are inherently dependent of data because instead of manual implementation of functionalities the ML systems learn those from data. 
    &
    Tools to manage data and visualize data dependency.
    \\
    
    Debugging  & All &
    Bugs might be in code as well as data. Debugging strategy of traditional systems are not quite applicable for many ML-systems. &
    Interpretable AI \cite{lipton2018mythos}\cite{ribeiro2016should} and debugging tools (MODE \cite{ma2018mode}). 
% MODE \cite{ma2018mode} is a debugging tool for identifying the internal features of the model that are responsible for the model's incorrect output. A deep learning model's bug can due to the sub-optimal model structure or biases in the data \cite{ma2018mode}. Model interpretability is known ML problem that signifies that the model's features are too abstract for human to understand\cite{lipton2018mythos}\cite{ribeiro2016should}\cite{lundberg2017unified}. A model is considered transparent if is by itself understandable.
    \\
    
    
    Immature workflow  &  All & 
    There is a lack of process management tools to estimate time and resources, ML-specific project maintenance, tools to identify \& report fault \cite{dlse_furute_2020}. 
    &
    Develop necessary specification and tools.
    \\
    
    Technical debt  &  All &
    A mature ML systems can be of 95\% of glue code that mainly connects different library and packages \cite{sculley_hiddent_debt_2015}\cite{SE_DL18}.
    &
    Develop methods and tools to report technical dependency. \\

    % ML applications accrue technical debt in many ways\cite{sculley_hiddent_debt_2015}. A mature ML systems can be of 95\% of glue code that mainly connects different library and packages \cite{sculley_hiddent_debt_2015}\cite{SE_DL18}. Transfer learning adds more external dependencies and cost of ownership. Currently the many other external systems or entity consumes the output of the ML model. These undeclared consumer systems can cause "visibility debt"\cite{morgenthaler2012searching} and can even cause hidden feedback loop.
    
    
     \midrule
    \textbf{Quality Assurance } & \\

    
    Test oracle spec. & Deployment & 
    Many MLSA's expected behaviours is not well defined and the model's performance is tested as a whole rather than for a specific input. So, it is challenging to design a test oracle \cite{barr2014oracle}. 
    &
    Research on better testing specification.
    \\

    Dependency analysis &  Deployment &
    If a ML model consume input features or delivers output for other systems then they become dependent on each other. This should be explicitly monitored because unlike code dependency data dependency is hard to detect\cite{sculley_hiddent_debt_2015}.
    &
    Develop Tools to detect code and data dependency\cite{sculley_hiddent_debt_2015}. 
    \\
    % ML applications are inherently dependent of data because instead of manual implementation of functionalities the ML systems learn those from data\cite{sculley_hiddent_debt_2015}. If a machine learning model consume input features from other systems or if other systems consume the output of the ML application then they become dependent on each other. This should be explicitly monitor because unlike code dependency data dependency is hard to detect. Various phases of a typical ML systems consists of highly coupled components data collection, cleaning, feature engineering, model design, execute and deployment. Faults occurred in one component of this pipeline propagate to other phase and it becomes hard to detect and fix\cite{sculley2014machine}. 
   
    
    Adversarial Robustness & Deployment \& monitoring &
    Adversarial example refers to a small malicious modification of the input that causes the model to erroneous output, while the change is imperceptible to a human. This phenomenon demonstrates that models are not learning the underlying concept of the problem in a robust manner \cite{madry2017towards}.
    % Adversarial example refers to a small malicious modification of the input that causes the model to erroneous output, while the change is imperceptible to a human. This phenomenon demonstrates that models are not learning the underlying concept of the problem in a robust manner \cite{madry2017towards}. Deep learning has made remarkable achievements in the computer vision domain and main research in adversarial attack and countermeasures are associated with this domain\cite{goodfellow2014explaining}\cite{carlini2017towards}\cite{szegedy2013intriguing}. There are also many novel adversarial attacks on deep neural networks\cite{dong2018boosting}\cite{carlini2017towards}. It is not common in real world scenarios but adversarial attacks can be carried out during model training by modifying the dataset or input features\cite{qiu2019review}. The attacks can be classified into two categories black-box and white-box attacks\cite{he2019towards}. The attacker can carry out white-box attack if he/she has access the algorithm, model parameters, and other necessary information. There are quite a few work proposing different adversarial attack \cite{szegedy2013intriguing, biggio2012poisoning, mei2015using} and defence mechanisms such as adversarial training\cite{goodfellow2014explaining, zhang2019defense}, defense distillation\cite{papernot2016distillation}, adversarial example detection\cite{carlini2017adversarial}, squeezing features \cite{he2017adversarial}, , transformation, gradient regularisation\cite{he2019towards}, gradient hiding\cite{tramer2017ensemble}, blocking transferability\cite{hosseini2017blocking}, data randomization\cite{xie2017adversarial}, data compression\cite{dziugaite2016study}, deep contractive network\cite{gu2014towards}. Auxiliary tools\cite{samangouei2018defense, meng2017magnet} can be used for defence.  
    & 
    Future research should focus more on black-box attacks and defence because in order to carry out this attack the attacker do not need to know about the target model\cite{qiu2019review}. 
    % Some of the defense mechanism proposed by the researchers have a good success rate at reducing attack severity but they are mostly aimed to prevent for a specific type of adversarial attack, rather than a general solution. Therefore, in order to ensure a robust and reliable ML technology researchers should explore the mentioned adversarial attack vectors and efficient defences. 
    \\
    
    Testing scope  & All &
    Data partly replaces code and both data and code should be considered during testing. & \\
    
    Testing approach & All &
    QA for ML systems are difficult because they are inherently non-deterministic, evolve over time with data i.e., self-learning. QA for ML-systems are not well defined\cite{borg2021aiq}\cite{lenarduzzi2021software} and it requires new QA approach from SE\cite{felderer_qa_overview_challenges_2021}.
    % QA is systematic way to ensure a software is operating under the designed specification. QA for ML systems are difficult because they are inherently non-deterministic, evolve over time with data, self-learning. So it requires new QA approach from SE\cite{felderer_qa_overview_challenges_2021}. QA for ML-systems are not well defined\cite{borg2021aiq}\cite{lenarduzzi2021software}. QA is crucial to increase trustworthiness for safely critical ML-applications such as self-driving cars (DeepXplore\cite{pei2017deepxplore}), medical tools. Oracle problem \cite{barr2014oracle} is very severe in ML. 
    & 
    % It is an emerging area that needs collaboration from SE and AI community. There are few research on testing model's accuracy and robustness but more research is needed on testing model's definition, specification of interpretability and relevance\cite{zhang_ml_testing_survey_horizons_2020}, bug analysis, regression testing. More research on unsupervised, transfer\cite{survey_transfer_learning_2009}, reinforced learning \cite{zhang_ml_testing_survey_horizons_2020}. Industry collaboration is needed for testing online models. Data testing is important\cite{amershi_se_case_study_2019}. There are some discussions on but not enough exploration on mutating machine learning code to better simulate real-world bugs \cite{zhang_ml_testing_survey_horizons_2020}\cite{cheng2018manifesting}. 
    \\
    
    
    Transparency &  All &
    Interpretability AI
    Model interpretability is known ML problem that signifies that the model's features are too abstract for human to understand\cite{lipton2018mythos}\cite{ribeiro2016should}\cite{lundberg2017unified}. 
    A deep learning model's bug can due to the sub-optimal model structure or biases in the data \cite{ma2018mode}.
    % Unlike a traditional software bug, a machine learning model's bug can not fixed easily by modifying the model. lack of understanding of misbehaviour. It is an active research area to understand when a model fails to make accurate prediction\cite{kulesza2015principles}.
    % MODE \cite{ma2018mode} is a debugging tool for identifying the internal features of the model that are responsible for the model's incorrect output. A deep learning model's bug can due to the sub-optimal model structure or biases in the data \cite{ma2018mode}. Model interpretability is known ML problem that signifies that the model's features are too abstract for human to understand\cite{lipton2018mythos}\cite{ribeiro2016should}\cite{lundberg2017unified}. A model is considered transparent if is by itself understandable.
    & 
    Model modularization\cite{pan2020decomposing} can provide a tiered software architecture widely applied in traditional software development can improve debuggability and maintainability.
    % Model modularization\cite{pan2020decomposing} can provide a tiered software architecture widely applied in traditional software development can improve debuggability and maintainability. One potential solutions is also to keep the humans in to loop to find model's "unknown unknown" problem \cite{attenberg2011beat}. 
    \\
    
    
    Biases \& fairness & All &
     This is a very broad and open issues. Unfairness can be found in both algorithms and data.
    % With the widespread use of ML in many sensitive environment it is high time to consider to ensure fairness into ML design. Many real world applications have shown biases\cite{mehrabi_fairness_survey_2019}\cite{o2016weapons}. Themis\cite{galhotra2017fairness} is a tool for detecting discrimination based on gender, race, marital status. There is still some challenges like what is the definition of fairness, should every group of people be given enough opportunity \cite{gooden2015race}\cite{mehrabi_fairness_survey_2019}. We should be careful of harmful usage of ML models like fake content generation\cite{kumar2017obamanet}. 
    & 
    Community detection and graph embedding is a fertile future research direction for studying biases and fairness\cite{mehrabi_fairness_survey_2019}.
    % This is a very broad and open issues. Unfairness can be found in algorithms, data, Natural language processing, classification problem etc. Different areas for fairness are not getting same level of research attention such as Community detection and graph embedding is a fertile future research direction for studying biases and fairness\cite{mehrabi_fairness_survey_2019}. 
    \\
    
    Reproducibility  & all &
    Many ML-libraries are random by nature and random data order, random initialization makes it hard to reproduce issues.
    &\\
    

    

    

    
 
  
    
    
    
    \midrule
    \textbf{Deployment }  & \\
    

    
    
    
    
    Devops support  & Deployment &
    There is a lack of tools that will help the teams to deploy the research experiment to the server with advanced logging, and automated roll back.
    & \\
    
    Compliance  & deployment &
    During deployment it should be tested if the model is exposing any sensitive data, or in violation of any compliance acts (HIPPA\cite{annas2003hipaa}, GDPR\cite{voigt2017eu}). &
    
    \\
    
    Scalability  & deployment &
    Many of the ML models perform well in research setting but not so well in real world in terms of accuracy and computational efficiency 
    &\\
    
    Configuration mngmt  & All &
    % There are many ML specific system configuration that needs to be tracked because the model's performance depends on it ML applications usually requires high maintenance specialized configuration.
    % & \\
    % Configuration Management & all &
    ML application contains code, data, parameters, hyperparameters. Rapid experimentation requires to track them to compare the trade-off of different algorithms, model architecture.  
    & \\
    
    

    
    
    
    
    \midrule
    \textbf{Maintenance } & \\
    Hidden feedback loop  & Monitoring &
    Data driven development, complex components, unspecified consumer of the model's output can cause hidden feedback loop. &
    \\
    % Configuration Management & all &
    % ML application contains code, data, parameters, hyperparameters. Rapid experimentation requires to track code, data, parameters, hyperparameters in-order to find the trade-off of different algorithms, model architecture.  
    % & \\
    
    Drift and decay & monitoring &
    ML systems have a predictable performance degradation and in order to ensure robustness models should be updated with new data in offline/online way &
    
    \\
    

    
    Model's robustness  & Monitoring &
    The deployed ML-application should perform reasonably on real world i.e., data it has not seen before or adversarial attacks\cite{schulam2019can}\cite{jiang2018trust} &
    \\
    Reliability monitoring & Monitoring &
    Once the system has been deployed, it requires monitoring to assess the output against new input. One potential approach is detecting out of distribution examples and reject it.
    % Once the system has been deployed, it requires monitoring to assess the output against new input. One potential approach is detecting out of distribution examples and reject it. These examples are not from the known training data distribution. This is known as anomaly detection or open-category detection. Apart from algorithmic solutions there are also approach for human-driven monitoring, human in the loop debugging approach \cite{saria_safe_reliable_2019}
    & 
    One way is to detect point wise trust score to predict whether to accept or reject the model's output\cite{schulam2019can}\cite{jiang2018trust}. We can consider the density principal and local fit principal for auditing\cite{saria_safe_reliable_2019}. 
    \\
    
    Technical debt  & All &
    Currently the many other external systems or entity consumes the output of the ML model. These undeclared consumer systems can cause "visibility debt"\cite{morgenthaler2012searching}.
    % ML applications accrue technical debt in many ways\cite{sculley_hiddent_debt_2015}. A mature ML systems can be of 95\% of glue code that mainly connects different library and packages \cite{sculley_hiddent_debt_2015}\cite{SE_DL18}. Transfer learning adds more external dependencies and cost of ownership. Currently the many other external systems or entity consumes the output of the ML model. These undeclared consumer systems can cause "visibility debt"\cite{morgenthaler2012searching} and can even cause hidden feedback loop. 
    &
    \\ 
    % \midrule
    % \textbf{ Miscellaneous } &  \\
    \bottomrule
    \end{tabular}%
%   }
   % \vspace{-.25in}
  \label{tab:mlsa_table}%
\end{table*}%










==> threats.tex <==
% \section{Threats to Validity}\label{subsec:validity}

